An FPGA Architecture for Online Learning using the Tsetlin Machine

There is a need for machine learning models to evolve in unsupervised circumstances. New classifications may be introduced, unexpected faults may occur, or the initial dataset may be small compared to the data-points presented to the system during normal operation. Implementing such a system using neural networks involves significant mathematical complexity, which is a major issue in power-critical edge applications. This paper proposes a novel field-programmable gate-array infrastructure for online learning, implementing a low-complexity machine learning algorithm called the Tsetlin Machine. This infrastructure features a custom-designed architecture for run-time learning management, providing on-chip offline and online learning. Using this architecture, training can be carried out on-demand on the \ac{FPGA} with pre-classified data before inference takes place. Additionally, our architecture provisions online learning, where training can be interleaved with inference during operation. Tsetlin Machine (TM) training naturally descends to an optimum, with training also linked to a threshold hyper-parameter which is used to reduce the probability of issuing feedback as the TM becomes trained further. The proposed architecture is modular, allowing the data input source to be easily changed, whilst inbuilt cross-validation infrastructure allows for reliable and representative results during system testing. We present use cases for online learning using the proposed infrastructure and demonstrate the energy/performance/accuracy trade-offs.

==> online-intro.tex <==
\subsection{Online Learning Overview}\label{sec:online-intro}
Traditional \ac{ML} models are trained before use leveraging an initial set of pre-classified data, so called \emph{batch learning}.
A recent concept has been to develop \ac{ML} models more akin to human learning, where the model learns over time and can develop to a variety of external changes.
This concept is called \emph{continual learning}, of which there are a variety of methods.
\emph{Online learning} \todo{SP:Make sure this is correct definition} involves training using data as it arrives at the system. Usually this data would only be used for inference, but online learning continues training.

\cite{delange2021continual}

==> pgflibraryshapes.gates.logic.comparator.code.tex <==
\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	comparator symbol/.initial=,
}

% Shape comparator
%
\pgfdeclareshape{comparator}{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@comparator\endcsname{%
    \pgf@lib@sh@logicgate@parseinputs{2}%
    \pgfmathloop%
    \ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
    \else%
            \pgfutil@ifundefined{pgf@anchor@comparator@input \pgfmathcounter}{%
                    \expandafter\xdef\csname pgf@anchor@comparator@input \pgfmathcounter\endcsname{%
                            \noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
                    }%
            }{}%
    \repeatpgfmathloop%
    \ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
      \pgferror{A comparator must have two inputs}%
    \fi%
  }%
  \savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
  \saveddimen\invertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
  }%
  \saveddimen\outerinvertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
          \advance\pgf@x.5\pgflinewidth%
  }
  \saveddimen\halflinewidth{%
    \pgf@x.5\pgflinewidth%
  }%
  \savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+0.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
    \midpoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{mid west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \midpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
    \basepoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{base west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \basepoint%
    \advance\pgf@x\pgf@xc%
  }%
  \inheritanchor[from=and gate US]{base}%
  \anchor{output}{%
    \dimensions%
    \pgf@xc\halfside%
    \centerpoint%
    \advance\pgf@x-.166666\pgf@xc%
    \pgf@xc2.0\pgf@xc%
    \advance\pgf@x.866025\pgf@xc%
    \advance\pgf@x\outerxsep%
  }%
  \anchor{east}{%
    \dimensions%
    \tipanchor%
    \pgf@xa\pgf@x%
    \centerpoint%
    \advance\pgf@x\pgf@xa%
  }%
  \anchor{north}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{north east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y-1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y-1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{north west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \centerpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \backgroundpath{%
    \dimensions%
    \pgf@xc\halfwidth%
    \pgf@yc\halfheight%
    \advance\pgf@xc-\outerxsep%
    \advance\pgf@yc-\outerysep%
    {%
	\pgftransformshift{\centerpoint}%
	\pgfpathmoveto{\tipanchor}%
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
	\pgfpathlineto{\tipanchor}%

	%
	% Draw inputs.
	%
	\pgf@xc-\halfwidth%
	\advance\pgf@xc-\invertedradius%
	\pgf@yc\halfheight%
	\pgfutil@tempdima2.0\pgf@yc%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\pgfmathloop%
	\ifnum\pgfmathcounter>\numinputs%
	\else%
		\advance\pgf@yc-\pgfutil@tempdima%
		\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
			{%
				\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
			}%
		\fi%
	\repeatpgfmathloop%
    }%
  }%
  \anchorborder{%
    \pgf@lib@gates@not@buffer@border{comparator}
  }%

}%


\endinput


==> pgflibraryshapes.gates.logic.mux.code.tex <==
% Copyright 2008 by Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	mux symbol/.initial=,
}

% Shape mux
%
\pgfdeclareshape{mux}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@mux\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@mux@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@mux@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A mux must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{mux}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}
	\anchor{mid west}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{mid east}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x\halfwidth}%
	\anchor{base}{\basepoint}
	\anchor{base west}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{base east}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x\halfwidth}%
	\anchor{north}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%
	\anchor{south}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%
	\anchor{east}{\dimensions\centerpoint\advance\pgf@x\halfwidth}%
	\anchor{west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth}%
	\anchor{north east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by -\pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{north west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y\halfheight}%
	\anchor{south east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by \pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{south west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y-\halfheight}%

	\anchor{select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%

	\anchor{other select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

  \backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\pgfmathaddtolength\pgf@xc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@yc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		{%
			\pgftransformshift{\centerpoint}%

      \pgfmathadd{\pgf@yc}{-1.155\pgf@xc}
      \let\pgf@yd\pgfmathresult

      \pgfpathmoveto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
			\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yd}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{-\pgf@yd}}
      \pgfpathclose

			%
			% Draw inputs.
			%
			\pgf@xc-\halfwidth%
			\advance\pgf@xc-\invertedradius%
			\pgf@yc\halfheight%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
					}%
				\fi%
			\repeatpgfmathloop%
		}%
  }

	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{mux}}

	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\dimensions%
		\pgfpointadd{\centerpoint}{\pgfpointborderrectangle{\externalpoint}{\pgfqpoint{\halfwidth}{\halfheight}}}%
	}%	

}


\endinput


==> texmf/tex/latex/common/pgflibraryshapes.gates.logic.comparator.code.tex <==
\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	comparator symbol/.initial=,
}

% Shape comparator
%
\pgfdeclareshape{comparator}{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@comparator\endcsname{%
    \pgf@lib@sh@logicgate@parseinputs{2}%
    \pgfmathloop%
    \ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
    \else%
            \pgfutil@ifundefined{pgf@anchor@comparator@input \pgfmathcounter}{%
                    \expandafter\xdef\csname pgf@anchor@comparator@input \pgfmathcounter\endcsname{%
                            \noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
                    }%
            }{}%
    \repeatpgfmathloop%
    \ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
      \pgferror{A comparator must have two inputs}%
    \fi%
  }%
  \savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
  \saveddimen\invertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
  }%
  \saveddimen\outerinvertedradius{%
          \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
          \advance\pgf@x.5\pgflinewidth%
  }
  \saveddimen\halflinewidth{%
    \pgf@x.5\pgflinewidth%
  }%
  \savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+0.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
    \midpoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{mid west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \midpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
    \basepoint%
    \pgfutil@tempdima\pgf@y%
    \csname pgf@anchor@comparator@east\endcsname%
    \pgf@y\pgfutil@tempdima%
  }%
  \anchor{base west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \basepoint%
    \advance\pgf@x\pgf@xc%
  }%
  \inheritanchor[from=and gate US]{base}%
  \anchor{output}{%
    \dimensions%
    \pgf@xc\halfside%
    \centerpoint%
    \advance\pgf@x-.166666\pgf@xc%
    \pgf@xc2.0\pgf@xc%
    \advance\pgf@x.866025\pgf@xc%
    \advance\pgf@x\outerxsep%
  }%
  \anchor{east}{%
    \dimensions%
    \tipanchor%
    \pgf@xa\pgf@x%
    \centerpoint%
    \advance\pgf@x\pgf@xa%
  }%
  \anchor{north}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \centerpoint%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@south west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y-1pt}%
      {\csname pgf@anchor@comparator@south west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{north east}{%
    \dimensions%
    \ifpgfgateanchorsuseboundingrectangle%
      \csname pgf@anchor@comparator@north west\endcsname%
      \pgf@ya\pgf@y%
      \pgf@process{%
        \dimensions%
        \tipanchor%
        \pgf@xa\pgf@x%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
      }%
      \pgf@y\pgf@ya%
    \else%
      \pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y1pt}%
      {\csname pgf@anchor@comparator@north west\endcsname}%
      {%
        \pgfpointadd{\centerpoint}{%
          \tipanchor%
          \pgf@xa\outerxsep%
          \advance\pgf@x2.350943\pgf@xa%
        }%
      }%
    \fi%
  }%
  \anchor{south west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y-1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y-1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{north west}{%
    \dimensions%
    \pgf@xa\halfside%
    \centerpoint%
    \advance\pgf@x-.833333\pgf@xa
    \advance\pgf@x-\outerxsep%
    \advance\pgf@y1.166666\pgf@xa%
    \pgf@ya\outerysep%
    \advance\pgf@y1.565\pgf@ya% Selected by trial and error.
  }%
  \anchor{west}{%
    \dimensions%
    \pgf@xc\halfside%
    \pgf@xc-.833333\pgf@xc%
    \advance\pgf@xc-\outerxsep%
    \centerpoint%
    \advance\pgf@x\pgf@xc%
  }%
  \backgroundpath{%
    \dimensions%
    \pgf@xc\halfwidth%
    \pgf@yc\halfheight%
    \advance\pgf@xc-\outerxsep%
    \advance\pgf@yc-\outerysep%
    {%
	\pgftransformshift{\centerpoint}%
	\pgfpathmoveto{\tipanchor}%
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
	\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
	\pgfpathlineto{\tipanchor}%

	%
	% Draw inputs.
	%
	\pgf@xc-\halfwidth%
	\advance\pgf@xc-\invertedradius%
	\pgf@yc\halfheight%
	\pgfutil@tempdima2.0\pgf@yc%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\pgfmathloop%
	\ifnum\pgfmathcounter>\numinputs%
	\else%
		\advance\pgf@yc-\pgfutil@tempdima%
		\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
			{%
				\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
			}%
		\fi%
	\repeatpgfmathloop%
    }%
  }%
  \anchorborder{%
    \pgf@lib@gates@not@buffer@border{comparator}
  }%

}%


\endinput


==> texmf/tex/latex/common/pgflibraryshapes.gates.logic.mux.code.tex <==
% Copyright 2008 by Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.gates.logic}
\usepgflibrary{shapes.gates.logic.IEC}

\pgfkeys{/pgf/.cd,
	mux symbol/.initial=,
}

% Shape mux
%
\pgfdeclareshape{mux}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@mux\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@mux@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@mux@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A mux must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{mux}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}
	\anchor{mid west}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{mid east}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x\halfwidth}%
	\anchor{base}{\basepoint}
	\anchor{base west}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{base east}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x\halfwidth}%
	\anchor{north}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%
	\anchor{south}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%
	\anchor{east}{\dimensions\centerpoint\advance\pgf@x\halfwidth}%
	\anchor{west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth}%
	\anchor{north east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by -\pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{north west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y\halfheight}%
	\anchor{south east}{%
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{1.155}%
    \advance\pgf@y by \pgfmathresult pt%
    \advance\pgf@x by \halfwidth%
  }%
	\anchor{south west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y-\halfheight}%

	\anchor{select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by -\halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by \pgfmathresult pt%
  }%

	\anchor{other select}{
    \dimensions%
    \centerpoint%
    \advance\pgf@y by \halfheight%
    \pgfmathmultiply{\halfwidth}{0.577}%
    \advance\pgf@y by -\pgfmathresult pt%
  }%

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 

  \backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\pgfmathaddtolength\pgf@xc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@yc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		{%
			\pgftransformshift{\centerpoint}%

      \pgfmathadd{\pgf@yc}{-1.155\pgf@xc}
      \let\pgf@yd\pgfmathresult

      \pgfpathmoveto{\pgfpoint{-\pgf@xc}{-\pgf@yc}}
			\pgfpathlineto{\pgfpoint{-\pgf@xc}{\pgf@yc}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yd}}
  		\pgfpathlineto{\pgfpoint{\pgf@xc}{-\pgf@yd}}
      \pgfpathclose

			%
			% Draw inputs.
			%
			\pgf@xc-\halfwidth%
			\advance\pgf@xc-\invertedradius%
			\pgf@yc\halfheight%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
					}%
				\fi%
			\repeatpgfmathloop%
		}%
  }

	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{mux}}

	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\dimensions%
		\pgfpointadd{\centerpoint}{\pgfpointborderrectangle{\externalpoint}{\pgfqpoint{\halfwidth}{\halfheight}}}%
	}%	

}


\endinput


==> texmf/tex/latex/common/tikzlibrarycircuits.logic.comparator.code.tex <==
\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.comparator}

\tikzset{
  circuit declare symbol = comparator,
}

\tikzset{
 set comparator graphic={
   circuit symbol open,
   circuit symbol size=width 0 height 4,
   shape=comparator,
   inner sep=.5ex
 }
}

\endinput


==> texmf/tex/latex/common/tikzlibrarycircuits.logic.mux.code.tex <==
% Copyright 2008 by Till Tantau and Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.mux}

\tikzset{
  circuit declare symbol = mux,
}

\tikzset{
 set mux graphic={
   circuit symbol open,
   circuit symbol size=width 2.5 height 6,
   shape=mux,
   inner sep=.5ex
 }
}

\endinput


==> texmf/tex/latex/common/tikzlibrarynicedash.code.tex <==
\usetikzlibrary{decorations, shapes.geometric}

% % https://tex.stackexchange.com/a/133357/132551
% \tikzset{
%     nice dash/.code args={on #1 off #2}{
%         % Use csname so catcode of @ doesn't have do be changed.
%         \csname tikz@addoption\endcsname{%
%             \pgfgetpath\currentpath%
%             \pgfprocessround{\currentpath}{\currentpath}%
%             \csname pgf@decorate@parsesoftpath\endcsname{\currentpath}{\currentpath}%
%             \pgfmathparse{\csname pgf@decorate@totalpathlength\endcsname-#1}\let\rest=\pgfmathresult%
%             \pgfmathparse{#1+#2}\let\onoff=\pgfmathresult%
%             \pgfmathparse{max(floor(\rest/\onoff), 1)}\let\nfullonoff=\pgfmathresult%
%             \pgfmathparse{max((\rest-\onoff*\nfullonoff)/\nfullonoff+#2, #2)}\let\offexpand=\pgfmathresult%
%             \pgfsetdash{{#1}{\offexpand}}{0pt}}%
%     }
% }

% https://tex.stackexchange.com/a/377390/132551
\makeatletter
\tikzset{%
  nice dash/.code args={on #1 off #2}{%
    \tikz@addoption{%
      \pgfgetpath\currentpath%
      \pgfprocessround{\currentpath}{\currentpath}%
      \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
      \pgfmathparse{max(round((\pgf@decorate@totalpathlength-#1)/(#1+#2)),0)}%
      \let\npattern=\pgfmathresult%
      \pgfmathparse{\pgf@decorate@totalpathlength/(\npattern*(#1+#2)+#1)}%
      \let\spattern=\pgfmathresult%
      \pgfsetdash{{\spattern*#1}{\spattern*#2}}{0pt}%
    }%
  }%
}
\makeatother


==> tikzlibrarycircuits.logic.comparator.code.tex <==
\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.comparator}

\tikzset{
  circuit declare symbol = comparator,
}

\tikzset{
 set comparator graphic={
   circuit symbol open,
   circuit symbol size=width 0 height 4,
   shape=comparator,
   inner sep=.5ex
 }
}

\endinput


==> tikzlibrarycircuits.logic.mux.code.tex <==
% Copyright 2008 by Till Tantau and Mark Wibrow
% Copyright 2015 by Gabi Sarkis
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{circuits.logic}
\usepgflibrary{shapes.gates.logic.mux}

\tikzset{
  circuit declare symbol = mux,
}

\tikzset{
 set mux graphic={
   circuit symbol open,
   circuit symbol size=width 2.5 height 6,
   shape=mux,
   inner sep=.5ex
 }
}

\endinput


==> tikzlibrarynicedash.code.tex <==
\usetikzlibrary{decorations, shapes.geometric}

% % https://tex.stackexchange.com/a/133357/132551
% \tikzset{
%     nice dash/.code args={on #1 off #2}{
%         % Use csname so catcode of @ doesn't have do be changed.
%         \csname tikz@addoption\endcsname{%
%             \pgfgetpath\currentpath%
%             \pgfprocessround{\currentpath}{\currentpath}%
%             \csname pgf@decorate@parsesoftpath\endcsname{\currentpath}{\currentpath}%
%             \pgfmathparse{\csname pgf@decorate@totalpathlength\endcsname-#1}\let\rest=\pgfmathresult%
%             \pgfmathparse{#1+#2}\let\onoff=\pgfmathresult%
%             \pgfmathparse{max(floor(\rest/\onoff), 1)}\let\nfullonoff=\pgfmathresult%
%             \pgfmathparse{max((\rest-\onoff*\nfullonoff)/\nfullonoff+#2, #2)}\let\offexpand=\pgfmathresult%
%             \pgfsetdash{{#1}{\offexpand}}{0pt}}%
%     }
% }

% https://tex.stackexchange.com/a/377390/132551
\makeatletter
\tikzset{%
  nice dash/.code args={on #1 off #2}{%
    \tikz@addoption{%
      \pgfgetpath\currentpath%
      \pgfprocessround{\currentpath}{\currentpath}%
      \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
      \pgfmathparse{max(round((\pgf@decorate@totalpathlength-#1)/(#1+#2)),0)}%
      \let\npattern=\pgfmathresult%
      \pgfmathparse{\pgf@decorate@totalpathlength/(\npattern*(#1+#2)+#1)}%
      \let\spattern=\pgfmathresult%
      \pgfsetdash{{\spattern*#1}{\spattern*#2}}{0pt}%
    }%
  }%
}
\makeatother

